Understanding the Difficulty of Training Transformers

Transformers have proved effective in many NLP tasks. However, their training requires non-trivial efforts regarding designing cutting-edge optimizers and learning rate schedulers carefully (e.g., conventional SGD fails to train Transformers effectively). Our objective here is to understand $\textit{what complicates Transformer training}$ from both empirical and theoretical perspectives. Our analysis reveals that unbalanced gradients are not the root cause of the instability of training. Instead, we identify an amplification effect that influences training substantially -- for each layer in a multi-layer Transformer model, heavy dependency on its residual branch makes training unstable, since it amplifies small parameter perturbations (e.g., parameter updates) and results in significant disturbances in the model output. Yet we observe that a light dependency limits the model potential and leads to inferior trained models. Inspired by our analysis, we propose Admin ($\textbf{Ad}$aptive $\textbf{m}$odel $\textbf{in}$itialization) to stabilize stabilize the early stage's training and unleash its full potential in the late stage. Extensive experiments show that Admin is more stable, converges faster, and leads to better performance. Implementations are released at: https://github.com/LiyuanLucasLiu/Transforemr-Clinic.

==> 7-con-short.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0--main.tex

\section{Conclusion}
Here, we study the difficulties of training Transformer in theoretical and empirical manners. 
We suggests that the gradient vanishing problem is not the root cause of the unstable Transformer training and this issue is largely addressed by adaptive optimizers. 
Besides, we reveal the root cause to be the strong dependency on residual branches, which amplifies the fluctuation and destabilizes model training. 
In light of our analysis, we propose \our, an adaptive initialization method to stabilize Transformers training. 
It controls the dependency in the early stage and maintains the flexibility to capture those dependencies once training stabilizes. 
Extensive experiments verify our intuitions and show \our gets more stable training, faster convergence, and better performance. 


==> old-3-ana-opt.tex <==

\section{Unbalanced Gradients}
\label{sec:gradient-distribution}

Here, we strive to answer the question: \emph{what complicates Transformer training}.
First, we observe that parts of parameters in Transformer have larger gradients than others. 
Here, we reveal that unbalanced gradients are caused by attention modules and hard to be neutralized. 
We observe this issue is largely addressed by adaptive optimizers and makes the vanilla SGD unsuited for Transformer training. 
Besides, we find this issue fails to explain the stability difference between Pre-LN and Post-LN, which implies the existance of other factors influencing Transformer training. 

\subsection{Attention Gradients}

As in Figure~\ref{fig:gradient-histogram} and Figure~\ref{fig:all_histogram}, the gradient distributions of Attention modules are unbalanced. 
Specifically, gradients of parameters within the softmax function (\ie, $\wk$ and $\wv$) have smaller gradients than parameters outside of the softmax function. 


Many attempts have been made to 

One distinguish character of Attention modules is its non-linear function. 
Different from conventional non-linear functions like ReLU or sigmoid, softmax has a dynamic input length (\ie, for sentence with different lengths, inputs of softmax have different dimensions). 
Although this setting allows Attention modules to handle sequential inputs, it also restricts them from having stable and consistent backpropagation. 
Specifically, let us consider the comparison between softmax and sigmoid. 
For the sigmoid function, although its derivation is smaller than 1, its damping ratio is consistent for all inputs. 
Thus, sigmoid can neutralize gradient vanishing by using a larger initialization~\cite{Glorot2010UnderstandingTD}. 
For softmax function, its damping ratio is different for input with different lengths (as shown in Figure~), which requires different initialization settings to neutralize the gradient vanishing/exploration.  
As only one initialization method can be used in practice, Attention modules would always lead to unbalanced gradients. 

To further verify our intuition, we visualize the relative gradient norm of self-attention modules 

Many attempts have been made to avoid gradient vanishing, which is able to hamper convergence from the beginning. 
For example, \citet{He2015DelvingDI} proposes an initialization schema to avoid gradient vanishing for backpropagation of ReLU activation functions. 
However, existing studies (introduced in Section~\ref{subsec:training-stable}) focuses on Linear networks, CNNs, and RNNs, but not Attention networks. 

\subsection{Effectiveness of Adaptive Optimizers}

Moreover, we find that even for Pre-LN Transformers, the gradient distribution is unbalanced. 
Specifically, $\wk$ and $\wq$ typically have a smaller gradient than other parameters, since their gradients are back-propagated through the softmax function. 
As in Figure, we first visualize the relative gradient norm of $\wk$, $\wq$, $\wv$ and $\wo$ in a 18-layer Pre-LN encoder (\ie, the gradient norm scaled by the largest norm in the same network) and find $|\Delta \wk|$ and $|\Delta \wq|$ could be smaller than $|\wv|$ and $|\wo|$ by more than one magnitude.
Moreover, we calculate the norm of parameter change in consequent epochs (\eg, $|\wk_{t+1} - \wk_{t}|$ where $\wk_{t}$ is the checkpoint saved after $t$ epochs) and also visualize the relative norm (scaled by the largest value in the same network) in Figure~\ref{fig:update-with-gradient}.  
Comparing the relative norm of parameter gradients and parameter updates, we notice that: although the gradient distribution is unbalanced, adaptive optimizers successfully assign different learning rates to different parameters and lead to consistent update magnitude. 
This results explains why the vanilla SGD fails for training Transformer (\ie, lacking the ability to handle unbalanced gradient distributions). 
Also, it implies that the unbalanced gradient distribution (\eg, gradient vanishing) has been largely addressed by existing techniques like adaptive optimizers (more discussions are included in Section~\ref{subsec:training-stable}) and may not have a big impact on the training instability. 

\subsection{Gradients at Initialization}
\label{subsec:ini_grad}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/all_and_postln_decoder_histogram.pdf}
\vspace{-0.5cm}
\caption{Relative gradient norm histogram of 18-layer Transformers on a log scale, \ie, the Frobenius norm of gradients of module/sub-layer outputs, scaled by the largest gradient norm in the same network. The default fairseq implementation is used~\cite{ott2019fairseq} and gradients are calculated on the first batch of WMT'14 En-De. }
\vspace{-0.3cm}
\label{fig:gradient-histogram}
\end{figure*}

As gradient vanishing is able to hamper convergence from the beginning, it has been long regarded as the major issue leading towards unstable training. 
Also, recent studies show this issue exists in the Post-LN Transformer, even after introducing residual connections to the network~\cite{Xiong2019OnLN}. 
Here, we first reveal Pre-LN does not suffer from the gradient vanishing. 
Then we establish that only the Post-LN decoder suffers from the gradient vanishing, but not the Post-LN encoder. 

$\Delta \xb$ is used to to denote gradients, \ie, $\Delta \xb = \frac{\partial \mathcal{L}}{\partial \xb}$ where $\mathcal{L}$ is the training objective. 
Following the previous study~\cite{Bengio1994LearningLD,Glorot2010UnderstandingTD,He2015DelvingDI,saxe2013exact}, we analyze the gradient distribution at the very beginning of training, assume that the randomly initialized parameters and the partial derivative of the module inputs are independent.
As established in Theorem~\ref{theo:post-ln-encoder-gradient} and Remark~\ref{remark: pre-ln-gradient}, both Post-LN Encoders and Pre-LN Encoders/Decoders do not suffer from gradient vanishing; it is only the Encoder-Attention layer in Post-LN suffer from gradient vanishing.  
Detailed derivations are included in Appendix~\ref{appendix:ini_grad}.

\begin{theorem}
For Post-LN Encoders, if $\bgamma$ and $\bnu$ are initialized as $1$ and $0$ respectively; all other parameters, 
% are initialized by symmetric distributions with zero mean; 
$\xb_{i}^{(oe)}$ and $\Delta \xb_i^{(oe)}$ subject to symmetric distributions with zero mean; $\Var[\xb_{i}^{(oe)}] = 1$ (\ie, normalized by Layer Norm); $\Delta \xb_i^{(oe)}$ and modules derivatives in the $i$-th sub-layer are independent, we have $\Var[\Delta \xb^{(oe)}_{i-1}] \geq \Var[\Delta \xb^{(oe)}_{i}]$.
\label{theo:post-ln-encoder-gradient}
\end{theorem}

\begin{remark}
For Pre-LN, if $\forall i, \Delta \xb_i^{(p\cdot)}$ and the derivatives of modules in the $i$-th sub-layer are independent, then $\forall i \leq j, \Var[\Delta \xb^{(p\cdot)}_{i}] \geq \Var[\Delta \xb^{(p\cdot)}_{j}]$.
\label{remark: pre-ln-gradient}
\end{remark}

Empirical studies are further conducted to verify Theorem~\ref{theo:post-ln-encoder-gradient} and Remark~\ref{remark: pre-ln-gradient}. 
% Specifically, 
At initialization, we calculate $||\Delta \xb^{(\cdot)}_{i}||_F$ for 18-layer Transformers\footnote{If $\E[\Delta \xb^{(p\cdot)}_{i-1}] = 0$, $\Var[\Delta \xb^{(p\cdot)}_{i-1}] \approx |\Delta \xb^{(p\cdot)}_{i-1}|_2^2$.} and visualize
$\frac{||\Delta \xb^{(\cdot)}_{i}||_F}{\max_j ||\Delta \xb^{(\cdot)}_{j}||_F}$ 
% are visualized 
in Figure~\ref{fig:gradient-histogram}.
As Theorem~\ref{theo:post-ln-encoder-gradient} and Remark~\ref{remark: pre-ln-gradient} meets the real-world observation, it verifies that it is only the Post-LN decoder suffers from the gradient vanishing. 
Also, it shows the gradient vanishing mainly happens in backpropagations from Encoder-Attention sub-layer outputs to its inputs (\ie, Self-Attention sub-layer outputs).

\subsection{Impact of the Gradient Vanishing}

Now we proceed to explore the impact of gradient vanishing. 
Firstly, we analyze whether gradient vanishing is the root cause of training instability.

\begin{table}[t]
\begin{center}
\small
\begin{tabularx}{\linewidth}{ *{4}{Y}}
\toprule
\textbf{Encoder} & \textbf{Decoder} & \textbf{Gradient} & \textbf{Training} \\ \midrule
Post-LN & Post-LN & Varnishing & Diverged \\
Post-LN & Pre-LN & \soutthick{Varnishing} & Diverged \\
Pre-LN & Pre-LN & \soutthick{Varnishing} & Converged \\
Admin & Admin & Varnishing & Converged \\
\bottomrule
\end{tabularx}
\end{center}
\vspace{-0.2cm}
\caption{Changing the decoder from Post-LN to Pre-LN fixes gradient vanishing, but does not stabilize model training successfully.}
\label{tbl:fixing-gradient-vanishing}
\vspace{-0.4cm}
\end{table}

As established in Section~\ref{subsec:ini_grad}, only Post-LN decoders suffer from gradient vanishing, but not Post-LN encoders. 
Thus, we combine Post-LN encoders with Pre-LN decoders to construct a hybrid Transformer, which does not suffer from gradient vanishing. 
As in Table~\ref{tbl:fixing-gradient-vanishing}, fixing the gradient vanishing alone (\ie, use Pre-LN decoder) fails to stabilize the model training. 
This phenomenon implies that the gradient vanishing is not the root cause of the unstable Transformer training. 


==> old-3-ana.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0--main.tex

\section{Unbalanced Gradient Distribution}
\label{sec:gradient-distribution}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/all_and_postln_decoder_histogram.pdf}
\vspace{-0.5cm}
\caption{Relative gradient norm histogram of 18-layer Transformers on a log scale, \ie, the Frobenius norm of gradients of module/sub-layer outputs, scaled by the largest gradient norm in the same network. The default fairseq implementation is used~\cite{ott2019fairseq} and gradients are calculated on the first batch of WMT'14 En-De. }
\vspace{-0.3cm}
\label{fig:gradient-histogram}
\end{figure*}

In this study, 
we strive to answer the question:
\emph{what makes Transformer training non-robust}.
We find that 
the root cause of this problem is not gradient vanishing, but the strong inter-layer dependency. 

\subsection{Gradients at Initialization}
\label{subsec:ini_grad}

As gradient vanishing is able to hamper convergence from the beginning, it has been long regarded as the major issue leading towards unstable training. 
Also, recent studies show this issue exists in the Post-LN Transformer, even after introducing residual connections to the network~\cite{Xiong2019OnLN}. 
Here, we first reveal Pre-LN does not suffer from the gradient vanishing. 
Then we establish that only the Post-LN decoder suffers from the gradient vanishing, but not the Post-LN encoder. 

For simplicity, we use $\Delta \xb$ to denote gradients, \ie, $\Delta \xb = \frac{\partial \mathcal{L}}{\partial \xb}$ where $\mathcal{L}$ is the training objective. 
Following the previous study~\cite{Bengio1994LearningLD,Glorot2010UnderstandingTD,He2015DelvingDI,saxe2013exact}, we analyze the gradient distribution at the very beginning of training, assume that the randomly initialized parameters and the partial derivative of the module inputs are independent.


\smallsection{Pre-LN Analysis}
For Pre-LN encoders, we have 
$ \xb\ep_{2i} = \xb\ep_{2i-1} + \FFN(\LN(\xb\ep_{2i-1}))$ and
$ \Delta\xb\ep_{2i-1} = \Delta\xb\ep_{2i} (1 + \frac{\partial \FFN(\LN(\xb\ep_{2i-1})) }{\partial \xb\ep_{2i}})$. 
At initialization, the two terms on the right part are approximately independent and $E[\frac{\partial \FFN(\LN(\zb\ep_{2i-1})) }{\partial \xb\ep_{2i}}] = 0$. Therefore we have $ \Var[\Delta\xb\ep_{2i-1}] \geq \Var[\Delta\xb\ep_{2i}]$.
Similarly, we can get $ \Var[\Delta\xb\ep_{2i-2}] \geq \Var[\Delta\xb\ep_{2i-1}]$ thus $\forall i \leq j, \Var[\Delta\xb\ep_{i}] \geq \Var[\Delta\xb\ep_{j}]$. 
Applying the same analysis to Pre-LN decoders, we can get $\forall i \leq j, \Var[\Delta\xb\pd_{i}] \geq \Var[\Delta\xb\pd_{j}]$.
Thus, lower layers have larger gradients than higher layers and gradients do not vanish in the back-propagation. 
\begin{remark}
For Pre-LN, if $\forall i, \Delta \xb_i^{(p\cdot)}$ and the derivatives of modules in the $i$-th sub-layer are independent, then $\forall i \leq j, \Var[\Delta \xb^{(p\cdot)}_{i}] \geq \Var[\Delta \xb^{(p\cdot)}_{j}]$.
\label{remark: pre-ln-gradient}
\end{remark}
We conduct empirical studies to verify Remark~\ref{remark: pre-ln-gradient}. 
At initialization, we calculate $||\Delta \xb^{(pe)}_{2i}||_F$ and $||\Delta \xb^{(pd)}_{3i}||_F$ for a 18-layer Pre-LN Transformer and visualize
$\frac{||\Delta \xb^{(pe)}_{2i}||_F}{\max_j ||\Delta \xb^{(pe)}_{2i}||_F}$
and $\frac{||\Delta \xb^{(de)}_{3i}||_F}{\max_j ||\Delta \xb^{(de)}_{3i}||_F}$ 
in Figure~\ref{fig:gradient-histogram}.
It
verifies that
the gradient norm does not vanish as propagating from top 
to bottom. 
Notice that if $\E[\Delta \xb^{(p\cdot)}_{i-1}] = 0$, $\Var[\Delta \xb^{(p\cdot)}_{i-1}] \approx |\Delta \xb^{(p\cdot)}_{i-1}|_2^2$.

\smallsection{Post-LN Encoder Analysis}
Different from Pre-LN, $\xb_{i}^{(oe)}$ and $\xb_{i-1}^{(oe)}$ are associated with not only the residual connection, but the layer normalization, which makes it harder to establish the connection on their gradients.
After making assumptions on the model initialization, we find that lower layers in Post-LN encoder also have larger gradients than higher layers and gradients do not vanish in the back-propagation through the encoder.   

\begin{theorem}
For Post-LN Encoders, if $\gamma$ and $\beta$ in the Layer Norm are initialized as $1$ and $0$ respectively; all other parameters are initialized by symmetric distributions with zero mean; $\xb_{i}^{(oe)}$ and $\Delta \xb_i^{(oe)}$ are subject to symmetric distributions with zero mean; the variance of $\xb_{i}^{(oe)}$ is $1$ (\ie, normalized by Layer Norm); $\Delta \xb_i^{(oe)}$ and the derivatives of modules in $i$-th sub-layer are independent, we have $\Var[\Delta \xb_{i-1}] \geq \Var[\Delta \xb_{i}]$.
\label{theo:post-ln-encoder-gradient}
\end{theorem}
\begin{proof}
We first analysis the backpropagation in the FFN sublayer, \ie, $\xb\eo_{2i} = \LN(\bbb\eo_{2i})$ where $\bbb\eo_{2i} =
\xb\eo_{2i-1} + \max(0, \xb\eo_{2i-1}\wf)\wff$.
Due to the symmetric and independent assumptions on parameters and inputs, we have $E[\bbb\eo_{2i}] = 0$. 
Thus, $\xb\eo_{2i} = \frac{\xb\eo_{2i-1} + \max(\xb\eo_{2i-1}\wf, 0)\wff}{\sigma_{b,2i}}$ where $\sigma_{b,2i}^2 = \Var[\bbb\eo_{2i}]$. 
Therefore, we have $\Var[\Delta \xb\eo_{2i-1}] \geq \Var[\frac{\Delta \xb\eo_{2i}}{\sigma_{b, 2i}} (1 + \frac{\partial \max(\xb\eo_{2i-1}\wf, 0)\wff}{\partial \xb\eo_{2i-1}})]$. 

As in the Appendix~\ref{appendix:theo1}, the full derivation establishes $ \Var[\frac{\partial \max(\xb\eo_{2i-1}\wf, 0)\wff}{\partial \xb\eo_{2i-1}}] + 1 = \sigma_{b,2i}^2$, which implies $\Var[\Delta \xb\eo_{2i-1}] \geq \Var[\Delta \xb\eo_{2i}]$. 
\end{proof}
Similar to Pre-LN, we also conduct empirical study for Post-LN encoders, visualize the relative gradient norm in Figure~\ref{fig:gradient-histogram} and find Theorem~\ref{theo:post-ln-encoder-gradient} meets the real-world observation. 

\smallsection{Post-LN Decoder Analysis}
In Post-LN, the Encoder-Attention sub-layer suffers from gradient vanishing. 
The Encoder-Attention sub-layer calculates outputs as 
$\xb\od_{3i-1} = \LN(\bbb\od_{3i-1})$ where $\bbb\od_{3i-1} = \xb\od_{3i-2} + \ab\od_{3i-1}$ and $\ab\od_{3i-1} = \sum_{h} \softmax(\xb\od_{3i-2} \wq_h \wk_h {\xb^T}^{(oe)})\xb^{(oe)} \wv_h \wo_h$. 
Here $\xb^{(oe)}$ is encoder outputs and $\softmax$ is the row-wise softmax function. 
In the backpropagation, $\Delta \xb\od_{3i-2} \approx \frac{\Delta \xb\od_{3i-1}}{\sigma_{b, 3i-1}} (1 + 
\frac{\partial \ab\od_{3i-1} }{\xb\od_{3i-2}}).$
All of backpropagations from $\ab\od_{3i-1} $ to $\xb\od_{3i-2}$ went through the softmax function, we have $\Var[\frac{\partial \ab\od_{3i-1} }{\xb\od_{3i-2}}] + 1 \leq \sigma^2_{b, 3i-1}$. 
Thus, those backpropagations suffer from gradient vanishing. 
Empirical studies are further conducted to verify the role of Encoder-Attention sublayers in the gradient vanishing. 
We visualize the relative gradient norm in Figure~\ref{fig:gradient-histogram}. 
Firstly, it verifies Post-LN decoder, unlike Pre-LN encoder/decoder and Post-LN encoder, suffers from the gradient vanishing. 
Also, it shows the gradient vanishing mainly happens in backpropagations from Encoder-Attention sub-layer outputs to its inputs (\ie, Self-Attention sub-layer outputs).

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig/self-attn-distribution-radam.pdf}
\caption{
Relative Gradient Norm and Relative Update Norm for Self-Attention Parameters in a 18-Layer Pre-LN Encoder. 
Darker color indicate bottom layers (smaller indexes) and light color indicate top layers (larger indexes). 
}
\vspace{-0.15cm}
\label{fig:update-with-gradient}
\vspace{-0.3cm}
\end{figure*}

\subsection{Impact of the Gradient Vanishing}

Now we proceed to explore the impact of gradient vanishing. 
Firstly, we analyze whether gradient vanishing is the root cause of training instability.

\begin{table}[t]
\begin{center}
\small
\begin{tabularx}{\linewidth}{ *{4}{Y}}
\toprule
\textbf{Encoder} & \textbf{Decoder} & \textbf{Gradient} & \textbf{Training} \\ \midrule
Post-LN & Post-LN & Varnishing & Diverged \\
Post-LN & Pre-LN & \soutthick{Varnishing} & Diverged \\
Pre-LN & Pre-LN & \soutthick{Varnishing} & Converged \\
\bottomrule
\end{tabularx}
\end{center}
\vspace{-0.2cm}
\caption{Changing the decoder from Post-LN to Pre-LN fixes gradient vanishing, but does not stabilize model training successfully.}
\label{tbl:fixing-gradient-vanishing}
\vspace{-0.4cm}
\end{table}


As established in Section~\ref{subsec:ini_grad}, only Post-LN decoders suffer from gradient vanishing, but not Post-LN encoders. 
Thus, we combine Post-LN encoders with Pre-LN decoders to construct a hybrid Transformer, which does not suffer from gradient vanishing. 
As in Table~\ref{tbl:fixing-gradient-vanishing}, fixing the gradient vanishing alone (\ie, use Pre-LN decoder) fails to stabilize the model training. 
This phenomenon implies that the gradient vanishing is not the root cause of the unstable Transformer training. 

Moreover, we find that even for Pre-LN Transformers, the gradient distribution is unbalanced. 
Specifically, $\wk$ and $\wq$ typically have a smaller gradient than other parameters, since their gradients are back-propagated through the softmax function. 
As in Figure~\ref{fig:update-with-gradient}, we first visualize the relative gradient norm of $\wk$, $\wq$, $\wv$ and $\wo$ in a 18-layer Pre-LN encoder (\ie, the gradient norm scaled by the largest norm in the same network) and find $|\Delta \wk|$ and $|\Delta \wq|$ could be smaller than $|\wv|$ and $|\wo|$ by more than one magnitude.
Moreover, we calculate the norm of parameter change in consequent epochs (\eg, $|\wk_{t+1} - \wk_{t}|$ where $\wk_{t}$ is the checkpoint saved after $t$ epochs) and also visualize the relative norm (scaled by the largest value in the same network) in Figure~\ref{fig:update-with-gradient}.  
Comparing the relative norm of parameter gradients and parameter updates, we notice that: although the gradient distribution is unbalanced, adaptive optimizers successfully assign different learning rates to different parameters and lead to consistent update magnitude. 
This results explains why the vanilla SGD fails for training Transformer (\ie, lacking the ability to handle unbalanced gradient distributions). 
Also, it implies that the unbalanced gradient distribution (\eg, gradient vanishing) has been largely addressed by adaptive optimizers and may not have a big impact on the training instability. 

